CAMP: Collaborative Attention Model with Profiles for Vehicle Routing Problems

The profiled vehicle routing problem (PVRP) is a generalization of the heterogeneous capacitated vehicle routing problem (HCVRP) in which the objective is to optimize the routes of vehicles to serve client demands subject to different vehicle profiles, with each having a preference or constraint on a per-client basis. While existing learning methods have shown promise for solving the HCVRP in real-time, no learning method exists to solve the more practical and challenging PVRP. In this paper, we propose a Collaborative Attention Model with Profiles (CAMP), a novel approach that learns efficient solvers for PVRP using multi-agent reinforcement learning. CAMP employs a specialized attention-based encoder architecture to embed profiled client embeddings in parallel for each vehicle profile. We design a communication layer between agents for collaborative decision-making across profiled embeddings at each decoding step and a batched pointer mechanism to attend to the profiled embeddings to evaluate the likelihood of the next actions. We evaluate CAMP on two variants of PVRPs: PVRP with preferences, which explicitly influence the reward function, and PVRP with zone constraints with different numbers of agents and clients, demonstrating that our learned solvers achieve competitive results compared to both classical state-of-the-art neural multi-agent models in terms of solution quality and computational efficiency. We make our code openly available at https://github.com/ai4co/camp.

==> _deprecated_chapters/old/1_introduction.tex <==
\section{Introduction}

\textbf{Contributions.} We summarize our contributions as follows:



\begin{itemize}
    \item We introduce \our{}.
\end{itemize}


==> _deprecated_chapters/old/2_preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Problem Formulation}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{example-image-b}
    \caption{Practical examples of PVRPs. [Left] PVRP-P has preference zones for each vehicle profile. [Right] PVRP-ZC has zone constraints that prevent certain vehicles from visiting.}
    \label{fig:pvrp-catchy}
\end{figure}

\paragraph{PVRP-P}

\paragraph{PVRP-ZC}


We show examples of PVRPs in \cref{fig:pvrp-catchy}.

==> _deprecated_chapters/old/3_method.tex <==
\section{Methodology}

\begin{figure*}
    \centering
    \includegraphics[width=.7\linewidth]{example-image-golden}
    \caption{\our{} Model}
    \label{fig:camp-model}
\end{figure*}

\subsection{RL Formulation for PVRP}

\subsection{Model} % i.e. the policy

\cref{fig:camp-model} shows the full \our{} model.

\subsubsection{Encoder}

\subsubsection{Decoder}

\subsection{Training}



==> _deprecated_chapters/old/4_experiments.tex <==
\section{Experiments}

\subsection{Experiments Setup}

\textit{Models} We evaluate neural methods that have been specifically designed to tackle the profile vehicle routing problems:

\begin{itemize}
    \item \texttt{ET} \needref
    \item \texttt{DPN} \needref
    \item \texttt{DRL} \needref
    \item \texttt{2D-Ptr} \needref
\end{itemize}

For fairness of comparison, we try to match the number of training steps to be the same and adjust the batch size accordingly. Specifically, we train models for 100 epochs as in \cite{kool2018attention} using the Adam optimizer \citep{kingma2014adam} with an initial learning rate (LR) of 0.001 with a decay factor of 0.1 after the 80th and 95th epochs with the SymNCO training scheme \cite{kim2022sym}. Every epoch, we sample $10^5$ samples. The policy gradients shared baseline is made of $8$ augmented symmetrical solutions out of a $128$-batch size.

\textit{Environment Settings} We evaluate the trained models under four types of environment settings:

\begin{itemize}
    \item \texttt{Random}: 
    \item \texttt{Angle}: 
    \item \texttt{Cluster}: 
    \item \texttt{Zone}: 
\end{itemize}

We emphasize open reproducibility and provide source code on Anonymous Github\footnote{\href{https://anonymous.4open.science/r/camp}{https://anonymous.4open.science/r/camp}}.

% \subsection{Quantitative Results}
\subsection{Experiment Results}


% TODO
\input{tables/placeholder}

\cref{table:hcvrp} \todo{placeholder} shows the main results for \our{}.


\textit{Quantitative analysis}. 

\textit{Qualitative analysis}. 

\subsection{Ablation Studies}


\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{example-image-a}
    \caption{Ablation studies}
    \label{fig:ablation-studies}
\end{figure}


\cref{fig:ablation-studies} illustrates the main ablation studies for the \our{} components.


\subsubsection{Collaborative Attention Layers} 
\label{subsec:collaborative-attention-layers}




\subsubsection{Balanced Reward Training} 
\label{subsec:balanced-reward-training}


==> _deprecated_chapters/old/5_relatedwork.tex <==
\section{Related Work}

% \paragraph{Multi-agent Construction Policies}

% \paragraph{NCO for Bi-objective Vehichle Routing Problems}


==> _deprecated_chapters/old/6_discussion_conclusion.tex <==
\section{Conclusion}

In this paper, we introduced a novel approach, \our{}.

==> tables/placeholder.tex <==
\begin{table*}[!t]
\centering
\caption{\todo{template - PVRP-P / PVRP-ZC if below} Benchmarks and results of our model for min-max HCVRP problems of varying sizes and agent numbers. Highlighting cost ($\downarrow$) and average gaps ($\downarrow$) from the best-known solutions of classical heuristic solvers. Inference times are shown in seconds in parentheses $(\cdot)$. (\textit{g.}) refers to greedy performance while (\textit{s.}) refers to sampling 1280 solutions.
}
\resizebox{\textwidth}{!}{%
    \begin{tabular}[\linewidth]{l| c c c | c c c | c c c | c}
    \toprule
    $N$ & \multicolumn{3}{c|}{60} & \multicolumn{3}{c|}{80} & \multicolumn{3}{c|}{100} & Gap($\%$)  \\
    \midrule
    % $m$ & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{7}  &\multicolumn{2}{c||}{10} &\multicolumn{2}{c}{5}  &\multicolumn{2}{c}{10} & \multicolumn{2}{c||}{15}  & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{15} & \multicolumn{2}{c||}{20} & - \\

    $m$ & 3 & 5 & 7 & 3 & 5 & 7 & 3 & 5 & 7 & avg.\\

        % & Cost & Time &  Cost & Time & Cost & Time & Cost & Time & Cost & Time & Cost & Time & Cost & Time & Cost & Time & Cost & Time & - \\
        
    \midrule
    
    % PRI & 8.32 & 6.23 & 4.64 & 15.43 & 7.89 & 5.84 & 14.35 & 10.11 & 8.01 & 346.29 \\
    SISR & 6.57 \small{(271)} & 4.00 \small{(274)}& 2.91 \small{(276)}& 8.52 \small{(425)}& 5.10\small{(430)} & 3.69 \small{(434)}
    & 10.29 \small{(615)} & 6.17 \small{(623)} & 4.45 \small{(625)} & 0.00 \\
    GA & 9.21 \small{(233)} & 6.89 \small{(320)} & 5.98 \small{(405)} & 12.32 \small{(347)}& 8.95 \small{(465)}& 7.58 \small{(578)}& 15.33 \small{(479)}& 10.93 \small{(623)}& 9.10 \small{(772)}& 74.90 \\
    SA & 7.04 \small{(130)}& 4.39 \small{(289)} & 3.30 \small{(362)}& 9.17 \small{(318)} & 5.61 \small{(417)} & 4.17 \small{(515)} & 11.13 \small{(434)}& 6.80 \small{(557)}& 5.01 \small{(678)}& 10.21 \\
    
    \midrule
    
    AM (\textit{g.}) & 8.49 \small{(0.08)} & 5.51 \small{(0.08)} & 4.15 \small{(0.09)} & 10.81 \small{(0.10)} & 6.87 \small{(0.11)}& 5.18 \small{(0.10)}& 12.68 \small{(0.14)}& 8.10 \small{(0.13)} & 6.13 \small{(0.13)} & 33.80 \\
    ET (\textit{g.}) & 7.58 \small{(0.15)}& 4.76 \small{(0.17)}& 3.58 \small{(0.16)} & 9.76 \small{(0.21)} & 6.01 \small{(0.20)}& 4.43 \small{(0.23)}& 11.74 \small{(0.25)} & 7.25 \small{(0.25)} & 5.23 \small{(0.26)} & 17.67 \\
    DRL$_{Li}$ (\textit{g.}) & 7.43 \small{(0.19)} & 4.71 \small{(0.22)} & 3.60 \small{(0.25)} & 9.64 \small{(0.25)} & 5.97 \small{(0.30)} & 4.52 \small{(0.33)}& 11.44 \small{(0.32)}& 7.06 \small{(0.37)} & 5.38 \small{(0.43)} & 17.08 \\
    2D-Ptr (\textit{g.}) & 7.20 \small{(0.11)} & 4.48 \small{(0.11)}& 3.31 \small{(0.11)} & 9.24 \small{(0.15)}& 5.65 \small{(0.15)}& 4.14 \small{(0.14)}& 11.12 \small{(0.18)}& 6.75 \small{(0.18)}& 4.92 \small{(0.17)}& 10.54 \\
    \our{} (\textit{g.}) & \textbf{7.12} \small{(0.12)}& \textbf{4.40} \small{(0.11)}& \textbf{3.25} \small{(0.11)}& \textbf{9.14} \small{(0.15)}& \textbf{5.53} \small{(0.15)}& \textbf{4.04} \small{(0.15)}& \textbf{10.98} \small{(0.19)} & \textbf{6.61} \small{(0.18)} & \textbf{4.79} \small{(0.18)}& 8.56 \\
    

    \midrule
    
    AM (\textit{s.}) & 7.62 \small{(0.14)} & 4.82 \small{(0.13)}& 3.63 \small{(0.14)}& 9.92 \small{(0.20)}& 6.19 \small{(0.21)}& 4.64 \small{(0.22)}& 11.82 \small{(0.29)}& 7.45 \small{(0.28)}& 5.58 \small{(0.28)}& 20.69 \\
    ET (\textit{s.}) & 7.14 \small{(0.21)}& 4.46 \small{(0.22)}& 3.33 \small{(0.22)}& 9.19 \small{(0.30)}& 5.64 \small{(0.30)}& 4.17 \small{(0.31)}& 11.20 \small{(0.41)}& 6.85 \small{(0.38)}& 4.98 \small{(0.40)}& 10.89 \\
    DRL$_{Li}$ (\textit{s.}) & 6.97 \small{(0.30)}& 4.34 \small{(0.36)}& 3.25 \small{(0.43)}& 9.10 \small{(0.45)}& 5.54 \small{(0.55)}& 4.13 \small{(0.65)}& 10.90 \small{(0.60)}& 6.65 \small{(0.76)}& 4.98 \small{(0.92)}& 8.78 \\
    2D-Ptr (\textit{s.}) & 6.82 \small{(0.13)}& 4.20 \small{(0.13)}& 3.09 \small{(0.14)}& 8.85 \small{(0.17)}& 5.36 \small{(0.18)}& 3.90 \small{(0.19)}& 10.71 \small{(0.22)}& 6.46 \small{(0.23)}& 4.68 \small{(0.24)}& 4.84 \\
    \our{} (\textit{s.}) & \textbf{6.82} \small{(0.31)} & \textbf{4.17} \small{(0.31)}& \textbf{3.06} \small{(0.31)}& \textbf{8.79} \small{(0.36)}& \textbf{5.28} \small{(0.36)}& \textbf{3.83} \small{(0.35)}& \textbf{10.61} \small{(0.40)}& \textbf{6.36} \small{(0.40)}& \textbf{4.58} \small{(0.40)}& 3.65 \\
    
    \bottomrule
    \end{tabular}
    }
\label{table:hcvrp}
\end{table*}






==> tables/pvrp-p.tex <==
\begin{table*}[ht!]
\centering
\caption{Benchmarks and results of our model for PVRP-P problems of varying sizes and agent numbers.  Highlighting cost ($\downarrow$) and average gaps ($\downarrow$) from the best-known solutions of classical heuristic solvers. Single instance solution time in $(\cdot)$.
% Highlighting cost ($\downarrow$) and average gaps ($\downarrow$) from the best-known solutions of classical heuristic solvers. Inference times are shown in parentheses $(\cdot)$. (\textit{g.}) refers to greedy performance while (\textit{s.}) refers to sampling 1280 solutions.
}
\resizebox{\textwidth}{!}{%
    \begin{tabular}[\linewidth]{l| c c c | c c c | c c c | c}
    \toprule
    $N$ & \multicolumn{3}{c|}{60} & \multicolumn{3}{c|}{80} & \multicolumn{3}{c|}{100} & Gap($\%$)  \\
    \midrule

    $m$ & 3 & 5 & 7 & 3 & 5 & 7 & 3 & 5 & 7 & avg.\\
        
    \midrule
    
    ORTools & 7.34 \small{(10m)} & 7.64 \small{(10m)} & 7.87 \small{(10m)} & 8.42 \small{(12m)} & 9.02 \small{(12m)} & 9.19 \small{(12m)} & 10.15 \small{(15m)} & 10.32 \small{(15m)} & 10.62 \small{(15m)} & 10.68 \\ 
    HGS     & 6.44 \small{(10m)} & 6.83 \small{(10m)} & 7.10 \small{(10m)} & 7.66 \small{(12m)} & 8.17 \small{(12m)} & 8.47 \small{(12m)} & 8.93 \small{(15m)} & 9.50 \small{(15m)} & 9.80 \small{(15m)} & 0.00 \\ 
    
    \midrule
    
    ET (\textit{g.}) & 7.62\small{(0.17s)} &8.12\small{(0.17s)} &8.41\small{(0.18s)} &9.04\small{(0.23s)} &9.63\small{(0.24s)} &9.96\small{(0.23s)} &10.50\small{(0.28s)} &11.18\small{(0.30s)} &11.63\small{(0.30s)} & 18.13\\
    DPN (\textit{g.}) & 7.52\small{(0.17s)} &8.00\small{(0.18s)} &8.27\small{(0.18s)} &8.93\small{(0.22s)} &9.63\small{(0.24s)} &10.05\small{(0.24s)} &10.50\small{(0.29s)} &11.08\small{(0.29s)} &11.42\small{(0.30s)} & 17.15\\
    2D-Ptr (\textit{g.}) & 7.34\small{(0.15s)} &7.75\small{(0.15s)} &8.03\small{(0.16s)} &8.70\small{(0.20s)} &9.30\small{(0.19s)} &9.59\small{(0.20s)} &10.10\small{(0.25s)} &10.82\small{(0.25s)} &11.18\small{(0.25s)} & 13.86\\
    PARCO (\textit{g.}) & 7.31\small{(0.14s)} &7.73\small{(0.15s)} &8.08\small{(0.15s)} &8.69\small{(0.21s)} &9.19\small{(0.22s)} &9.57\small{(0.22s)} &10.14\small{(0.25s)} &10.78\small{(0.24s)} &11.10\small{(0.25s)} & 13.21\\
    \our{}(-EC) (\textit{g.}) & 7.30\small{(0.16s)} & 7.67\small{(0.15s)} & 7.90\small{(0.16s)} & 8.68\small{(0.22s)} & 9.10\small{(0.21s)} & 9.49\small{(0.21s)} & 9.98\small{(0.25s)} & 10.72\small{(0.25s)} & 11.00\small{(0.26s)} & 12.53\\
    \our{} (\textit{g.}) & \textbf{7.16}\small{(0.17s)} &\textbf{7.66}\small{(0.18s)} & \textbf{7.88}\small{(0.18s)} & \textbf{8.49}\small{(0.25s)} & \textbf{9.07}\small{(0.25s)} & \textbf{9.44}\small{(0.25s)} & \textbf{9.87}\small{(0.33s)} & \textbf{10.60}\small{(0.33s)} & \textbf{10.90}\small{(0.33s)} & \textbf{11.23}\\
    
    \midrule
    
    ET (\textit{s.}) & 7.16\small{(0.25s)} &7.62\small{(0.24s)} &7.87\small{(0.25s)} &8.51\small{(0.35s)} &9.05\small{(0.37s)} &9.41\small{(0.36s)} &9.93\small{(0.45s)} &10.55\small{(0.44s)} &10.88\small{(0.46s)} & 11.23\\
    DPN (\textit{s.}) & 7.13\small{(0.27s)} &7.55\small{(0.26s)} &7.87\small{(0.26s)} &8.46\small{(0.34s)} &9.04\small{(0.37s)} &9.36\small{(0.36s)} &9.85\small{(0.43s)} &10.52\small{(0.42s)} &10.88\small{(0.48s)} & 10.69\\
    2D-Ptr (\textit{s.}) & 6.89\small{(0.16s)} &7.31\small{(0.17s)} &7.57\small{(0.17s)} &8.23\small{(0.20s)} &8.72\small{(0.21s)} &9.09\small{(0.22s)} &9.57\small{(0.26s)} &10.14\small{(0.26s)} &10.45\small{(0.27s)} & 6.81\\
    PARCO (\textit{s.}) & 6.87\small{(0.21s)} &7.25\small{(0.23s)} &7.55\small{(0.22s)} &8.13\small{(0.33s)} &8.66\small{(0.35s)} &9.02\small{(0.34s)} &9.44\small{(0.42s)} &10.12\small{(0.41s)} &10.49\small{(0.41s)} & 6.44\\
    \our{}(-EC) (\textit{s.}) & 6.82\small{(0.22s)} & 7.20\small{(0.23s)} & 7.54\small{(0.23s)} & 8.12\small{(0.33s)} & 8.63\small{(0.32s)} & 8.95\small{(0.34s)} & 9.42\small{(0.40s)} & 10.05\small{(0.42s)} & 10.32\small{(0.41s)} & 5.72\\
    \our{} (\textit{s.}) &\textbf{ 6.75}\small{(0.33s)} &\textbf{7.18}\small{(0.35s)} &\textbf{7.45}\small{(0.33s)} &\textbf{8.05}\small{(0.43s)} &\textbf{8.57}\small{(0.42s)} &\textbf{8.90}\small{(0.42s)} &\textbf{9.38}\small{(0.51s)} &\textbf{9.96}\small{(0.54s)} &\textbf{10.29}\small{(0.54s)} & \textbf{5.02}\\
    
    \bottomrule
    \end{tabular}
    }
\label{table:pvrp-p}
\end{table*}






==> tables/pvrp-zc.tex <==
\begin{table*}[ht!]
\centering
\caption{Benchmarks and results of our model for PVRP-ZC problems of varying sizes and agent numbers.  Highlighting cost ($\downarrow$) and average gaps ($\downarrow$) from the best-known solutions of classical heuristic solvers. Single instance solution time in $(\cdot)$.
}
\resizebox{\textwidth}{!}{%
    \begin{tabular}[\linewidth]{l| c c c | c c c | c c c | c}
    \toprule
    $N$ & \multicolumn{3}{c|}{60} & \multicolumn{3}{c|}{80} & \multicolumn{3}{c|}{100} & Gap($\%$)  \\
    \midrule

    $m$ & 3 & 5 & 7 & 3 & 5 & 7 & 3 & 5 & 7 & avg.\\
        
    \midrule
    
    ORTools & 13.17\small{(10m)} & 13.15\small{(10m)} & 13.18\small{(10m)} & 16.67\small{(12m)} & 16.69\small{(12m)} & 16.70\small{(12m)} & 20.18\small{(15m)} & 20.22\small{(15m)} & 20.20\small{(15m)} & 8.35\\
    HGS & 12.13\small{(10m)} & 12.16\small{(10m)} & 12.16\small{(10m)} & 15.36\small{(12m)} & 15.40\small{(12m)} & 15.42\small{(12m)} & 18.59\small{(15m)} & 18.66\small{(15m)} & 18.70\small{(15m)} & 0.00\\
    
    \midrule
    
    ET (\textit{g.}) & 13.87\small{(0.17s)} & 14.04\small{(0.17s)} & 13.91\small{(0.17s)} & 17.55\small{(0.23s)} & 17.54\small{(0.23s)} & 17.48\small{(0.24s)} & 21.28\small{(0.28s)} & 21.20\small{(0.29s)} & 21.36\small{(0.29s)} & 14.15\\
    DPN (\textit{g.}) & 13.98\small{(0.17s)} & 13.94\small{(0.17s)} & 13.81\small{(0.17s)} & 17.50\small{(0.22s)} & 17.62\small{(0.22s)} & 17.57\small{(0.23s)} & 21.24\small{(0.28s)} & 21.31\small{(0.28s)} & 21.37\small{(0.28s)} & 14.14\\
    2D-Ptr (\textit{g.}) & 13.42\small{(0.15s)} & 13.49\small{(0.15s)} & 13.37\small{(0.15s)} & 16.98\small{(0.20s)} & 16.95\small{(0.20s)} & 17.04\small{(0.20s)} & 20.53\small{(0.25s)} & 20.58\small{(0.24s)} & 20.57\small{(0.25s)} & 10.06\\
    PARCO (\textit{g.}) & 13.39\small{(0.14s)} & 13.42\small{(0.13s)} & 13.32\small{(0.13s)} & 16.87\small{(0.21s)} & 16.95\small{(0.20s)} & 16.82\small{(0.20s)} & 20.33\small{(0.25s)} & 20.52\small{(0.25s)} & 20.33\small{(0.25s)} & 9.55\\
    \our{}(-EC) (\textit{g.}) & 13.05\small{(0.17s)} & 13.19\small{(0.16s)} & \textbf{13.05}\small{(0.16s)} & \textbf{16.58}\small{(0.22s)} & 16.73\small{(0.23s)} & 16.65\small{(0.22s)} & 20.10\small{(0.25s)} & \textbf{20.07}\small{(0.25s)} & 20.07\small{(0.26s)} & 7.69\\
    \our{} (\textit{g.}) & \textbf{12.93}\small{(0.19s)} & \textbf{13.07}\small{(0.20s)} & 13.14\small{(0.18s)} & 16.59\small{(0.25s)} & \textbf{16.38}\small{(0.25s)} & \textbf{16.52}\small{(0.24s)} & \textbf{20.00}\small{(0.33s)} & 20.18\small{(0.32s)} & \textbf{20.07}\small{(0.33s)} & \textbf{7.62}\\
    
    \midrule
    
    ET (\textit{s.}) & 13.18\small{(0.25s)} & 13.17\small{(0.25s)} & 13.18\small{(0.25s)} & 16.63\small{(0.34s)} & 16.73\small{(0.34s)} & 16.58\small{(0.34s)} & 20.19\small{(0.46s)} & 20.47\small{(0.45s)} & 20.14\small{(0.45s)} & 8.78\\
    DPN (\textit{s.}) & 13.13\small{(0.27s)} & 13.30\small{(0.27s)} & 13.24\small{(0.26s)} & 16.62\small{(0.33s)} & 16.67\small{(0.33s)} & 16.78\small{(0.34s)} & 20.23\small{(0.44s)} & 20.18\small{(0.44s)} & 20.34\small{(0.43s)} & 8.69\\
    2D-Ptr (\textit{s.}) & 12.86\small{(0.15s)} & 12.93\small{(0.15s)} & 12.99\small{(0.15s)} & 16.33\small{(0.21s)} & 16.31\small{(0.21s)} & 16.17\small{(0.22s)} & 19.76\small{(0.25s)} & 19.72\small{(0.25s)} & 19.90\small{(0.25s)} & 5.92\\
    PARCO (\textit{s.}) & 12.85\small{(0.21s)} & 12.81\small{(0.22s)} & 12.86\small{(0.22s)} & 16.28\small{(0.33s)} & 16.46\small{(0.33s)} & 16.31\small{(0.33s)} & 19.64\small{(0.42s)} & 19.72\small{(0.42s)} & 19.79\small{(0.41s)} & 5.86\\
    \our{}(-EC) (\textit{s.}) & \textbf{12.49}\small{(0.22s)} & 12.58\small{(0.23s)} & 12.56\small{(0.23s)} & 15.87\small{(0.33s)} & 15.92\small{(0.32s)} & \textbf{15.86}\small{(0.33s)} & 19.20\small{(0.41s)} & \textbf{19.19}\small{(0.41s)} & 19.18\small{(0.40s)} & 3.34\\
    \our{} (\textit{s.}) & 12.54\small{(0.33s)} & \textbf{12.50}\small{(0.33s)} & \textbf{12.52}\small{(0.34s)} & \textbf{15.77}\small{(0.42s)} & \textbf{15.84}\small{(0.43s)} & 15.88\small{(0.42s)} & \textbf{19.06}\small{(0.50s)} & 19.26\small{(0.49s)} & \textbf{19.18}\small{(0.49s)} & \textbf{3.31}\\    
    
    \bottomrule
    \end{tabular}
    }
\label{table:pvrp-zc}
\end{table*}

